Scaling Law Phenomena Across Regression Paradigms: Multiple and Kernel Approaches

Recently, Large Language Models (LLMs) have achieved remarkable success. A key factor behind this success is the scaling law observed by OpenAI. Specifically, for models with Transformer architecture, the test loss exhibits a power-law relationship with model size, dataset size, and the amount of computation used in training, demonstrating trends that span more than seven orders of magnitude. This scaling law challenges traditional machine learning wisdom, notably the Oscar Scissors principle, which suggests that an overparametrized algorithm will overfit the training datasets, resulting in poor test performance. Recent research has also identified the scaling law in simpler machine learning contexts, such as linear regression. However, fully explaining the scaling law in large practical models remains an elusive goal. In this work, we advance our understanding by demonstrating that the scaling law phenomenon extends to multiple regression and kernel regression settings, which are significantly more expressive and powerful than linear methods. Our analysis provides deeper insights into the scaling law, potentially enhancing our understanding of LLMs.

==> 5_kernel_regression.tex <==


\section{Main Results}

In this section, we introduce our main results.
In Section~\ref{sec:scaling_law_multiple}, we present the scaling law and its generalization error bounds for multiple regression. 
In Section~\ref{sec:scaling_law_kernel}, we present the scaling law and its generalization error bounds for kernel regression.

\subsection{Scaling law for Multiple Regression}\label{sec:scaling_law_multiple}

In this section, we present the scaling law for multiple regression and introduce the assumptions necessary for our results.

\begin{assumption}[Gaussianity]\label{ass:gaussian_feature}
    Assume that $(x, y)$ drawn from $P$ satisfies $x \sim \N(0, G)$.
\end{assumption}

Assumption \ref{ass:gaussian_feature} establishes the distributional properties of the feature mapping, which will facilitate subsequent analysis under the Gaussian framework.


\begin{assumption}[Well-specified Multiple Regression Model]\label{ass:well_specified}
    Assume that $(x, y)$ drawn from $P$ satisfy $\E_{ (x,y) \sim P }[y~|~x]=W^{*\top}x$. Define $\sigma^2 := \E_{(x,y)\sim P}[\|y-W^{*\top}x \|_2^2]$.
\end{assumption}

Assumption \ref{ass:well_specified} introduces the well-specified nature of the feature mapping, ensuring that the target $y$ is conditionally linear in $\phi(x)$, which aids in specifying the true parameter $W^*$.


\begin{assumption}[Parameter Prior]\label{ass:parameter_prior}
    Assume that $W^*$ satisfies a prior such that $\E[W^* W^{*\top}] = I_{d\times d}$.
\end{assumption}

This prior assumption on $W^*$ ensures that the covariance of the parameter vector is well-structured, which will be critical for deriving the posterior distribution.

\begin{assumption}[Power Law Spectrum]\label{ass:power_law_spectrum:kernel}
    There exists $a > 1$ such that the eigenvalues of $G$ satisfy $\lambda_i = \Theta(i^{-a}), i > 0$.
\end{assumption}

Assumption \ref{ass:power_law_spectrum:kernel} constrains the spectrum of the feature covariance matrix, implying a power law decay for the eigenvalues, which characterizes the complexity of the feature space.

Building upon the established assumptions and setup, we present our main theoretical result regarding the generalization error bounds under the sketched predictor scenario.

\begin{theorem}[Generalization Error Bounds for Multiple Regression Scaling Law]\label{thm:error_multiregression}
If the following conditions hold:
\begin{itemize}
    \item Suppose that Assumptions~\ref{ass:gaussian_feature}, \ref{ass:well_specified}, \ref{ass:parameter_prior}, and \ref{ass:power_law_spectrum:kernel} hold.
    \item Consider an $m$-dimensional sketched predictor trained by (SGD Lemma~\ref{lem:multi_sgd}) with $n$ samples.
     \item Let $\neff := n/ \log(n )$ and recall the generalization error decomposition in Lemma~\ref{lem:risk_decompose}.
    \item Let $D = \{(x_1, y_1), (x_2, y_2), \ldots, (x_n, y_n)\}$ be the sample set i.i.d. drawn from $P$.
    \item Let the initial stepsize $\gamma \leq c$ for some $a$-dependent constant $c > 0$.
\end{itemize}   
   Then with probability at least $1 - e^{-\Omega(M )}$ over the randomness of the sketch matrix $R$, we have
\begin{itemize}
    \item Part 1. $\irre = \sigma^2$.
    \item Part 2. $\E_{W^*}[\appr] = \Theta(m^{1-a})$.
\end{itemize}
    If we further assume that $\sigma^2 = \Omega(1)$, then the following holds
\begin{itemize}
    \item Part 3. $  \E_{W^*}[\E_{D \sim P^n}[\excess]] = \Theta (\bias + \sigma^2 \vari). $   
\end{itemize}
\end{theorem}

\begin{proof}
    {\bf Part 1.} 
    First we show,
    \begin{align*}
        \loss(W) 
        = & ~ \E[\| W^\top x - y \|_2^2] \\
        = & ~ \E[ \| (W^\top - W^{*\top})x + (W^{*\top}x-y) \|_2^2 ] \\
        = & ~ \E[ \| (W^\top - W^{*\top})x \|_2^2 + \|(W^{*\top}x-y) \|_2^2 ] \\
        \geq & ~ \sigma^2
    \end{align*}
    where the first step follows from Definition~\ref{def:multiple_regression_sketching}, the second step follows from basic algebra, the third step follows from the definition of $\ell_2$-norm, and the fourth step follows from Assumption~\ref{ass:well_specified} and $\ell_2$-norm $\geq 0$.

    {\bf Part 2.} Follows from Lemma~\ref{lem:approx_error_lower_bound_mutliregression}.

    {\bf Part 3.} Follows from Lemma~\ref{lem:excee_risk_bounds}
    
\end{proof}

Theorem \ref{thm:error_multiregression} provides a comprehensive characterization of the generalization performance, revealing how the error decomposes based on various structural assumptions and conditions of the predictor. This result highlights key dependencies on parameters such as the sketch dimension $M$, the effective sample size $N_{\rm eff}$, and the feature spectrum.

Leveraging the generalization error bounds established in Theorem \ref{thm:error_multiregression}, we derive a scaling law that provides further insights into how the error components behave under different parameter regimes.

\begin{theorem}[Scaling Law for Multiple Regression]\label{thm:main}
    Assume all conditions in Theorem~\ref{thm:error_multiregression} hold. Then with probability at least $1 - e^{-\Omega(M )}$ over the randomness of the sketch matrix $R$ that
    \begin{align*}
      \E[\loss_R(V_n)]] = \sigma^2 + \Theta(\frac{1}{M^{a-1}}) + \Theta(\frac{1}{(N_{\rm eff} \gamma)^{(a-1)/a}}).
    \end{align*}
\end{theorem}

\begin{proof}
    Adding all the errors in Theorem~\ref{thm:error_multiregression}, we can derive the scaling law.
\end{proof}

Theorem \ref{thm:main} reveals the interplay between the sketch dimension $M$, the effective sample size $\neff$, and the learning rate $\gamma$ in determining the overall loss, offering a practical guideline for scaling behavior in sketched predictors.

\subsection{Scaling Law for Kernel Regression}\label{sec:scaling_law_kernel}

In this section, we provide the generalization error bounds for kernel regression scaling law. We just need to replace the sketching $\|V^\top (Rx) - y \|_2^2$ from Definition~\ref{def:multiple_regression_sketching} with $(\langle R\phi(x),v\rangle-y)^2$ in proofs of Lemma~\ref{lem:approximation_error:multiregression},~\ref{lem:approx_error_upper_bound_mutliregression},~\ref{lem:approx_error_lower_bound_mutliregression},~\ref{lem:bias_error_upper_bound_mutliregression} ,~\ref{lem:bias_error_lower_bound_mutliregression},~\ref{lem:hypercontractivity and misspecified noise},~\ref{lem:gaussianity and noise},~\ref{lem:excee_risk_bounds}


\begin{corollary}[Generalization Error Bounds for Kernel Regression Scaling Law]\label{cor:gaussianity:kernel}
If the following conditions hold:
\begin{itemize}
    \item Assume that $(x, y)$ drawn from $P$ and the feature mapping $\phi$ satisfy $\phi(x) \sim \N(0, \Phi)$.
    \item Assume that $(x, y)$ drawn from $P$ and the feature mapping $\phi$ satisfy $\E_{ (x,y) \sim P }[y~|~x]=\phi(x)^\top w^*$. Define $\sigma^2 := \E_{(x,y)\sim P}[(y-\phi(x)^\top w^*)^2]$.
\end{itemize}
Then the following statements hold:
\begin{itemize}
    \item Part 1. $R\phi(x) \sim \N(0, R\Phi  R^\top)$.
    \item Part 2. $\E [y ~ |~ R \phi(x)] = \langle R\phi(x),V^*\rangle$.
    \item Part 3. $\E[(y- \langle R\phi(x),V^*\rangle)^2] = \sigma^2 + \appr \geq \sigma^2$.
\end{itemize}
\end{corollary}
\begin{proof}[Proof Sketch]
    Proof is similar to the multiple regression proof in Theorem~\ref{thm:error_multiregression} by using Definition~\ref{def:regression_sketch:kernel}.
\end{proof}



